Beyond Performance: Quantifying and Mitigating Label Bias in LLMs

Large language models (LLMs) have shown remarkable adaptability to diverse tasks, by leveraging context prompts containing instructions, or minimal input-output examples. However, recent work revealed they also exhibit label bias -- an undesirable preference toward predicting certain answers over others. Still, detecting and measuring this bias reliably and at scale has remained relatively unexplored. In this study, we evaluate different approaches to quantifying label bias in a model's predictions, conducting a comprehensive investigation across 279 classification tasks and ten LLMs. Our investigation reveals substantial label bias in models both before and after debiasing attempts, as well as highlights the importance of outcomes-based evaluation metrics, which were not previously used in this regard. We further propose a novel label bias calibration method tailored for few-shot prompting, which outperforms recent calibration approaches for both improving performance and mitigating label bias. Our results emphasize that label bias in the predictions of LLMs remains a barrier to their reliability.

==> figures/imbalanced_labels/fig.tex <==
\begin{figure}[!t]
    \centering
    \captionsetup[subfigure]
    {font=small,labelfont=small} %,aboveskip=-5pt} % ,font=tiny,labelfont=tiny
    
    \begin{subfigure}[t]{0.67\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/imbalanced_labels/src/All_rsd.png}%
        
        \subcaption{\rsd}\label{fig:imbalanced_labels_RSD}%
    \end{subfigure}%
\vspace{2mm}
    \begin{subfigure}[t]{0.67\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/imbalanced_labels/src/All_bias_score.png}%
        \subcaption{\bias}\label{fig:imbalanced_labels_BiasScore}%
    \end{subfigure}%
\vspace{2mm}
    \begin{subfigure}[t]{0.67\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{figures/imbalanced_labels/src/All_macro_f1.png}%
        
        \subcaption{\textsl{Macro-F1}}\label{fig:imbalanced_labels_F1}%
    \end{subfigure}%
    \caption{Label bias and performance metrics for Llama-2 (7B/13B) and Mistral (7B) models, when aggregated by the level of imbalance in the demonstrations set used for prompting the model, measured by the proportions of its most frequent label ($p_\uparrow$). For most tasks, label imbalance has only minor impact on both bias and performance, unless the imbalance is extreme. Instruction-tuned models are less sensitive to imbalance.
    }
    
    % \caption{\yuval{Performance and label bias measures for calibration methods (CC - yellow, DC - pink. No calibration - grey/black). Again we have contradictions between Bias Score and RSD and performance, pretty much the same ones. Findings: 1. for all models, CC can sometimes slightly improve performance or bias, but hurts performance for instruction-tuned models (except for Falcon-7B). This is also shown in both bias metrics 2. For zero-shot/few-shot with very few demonstrations (2-4), calibration with DC often substantially improves both performance and bias. 3. However, for instruction tuned-models (dashed lines) with 8 or more demonstrations, calibration mostly doesn't help much for performance, and neither for removing bias (RSD).}}
\label{fig:imbalanced_labels}
\end{figure}

